Prescribed Performance Guided Safe Reinforcement Learning for Roundabout Navigation of Autonomous Vehicles

Connected and Autonomous Vehicles (CAVs) face significant challenges in roundabout navigation due to dense traffic interactions and unpredictable agent behaviors, necessitating high levels of adaptability and safety. While the combination of Reinforcement Learning (RL) and Model Predictive Control (MPC) offers a promising approach, existing frameworks suffer from a structural mismatch where pointwise RL decisions fail to align with MPC's trajectory level optimization, and often lack rigorous safety guarantees. This work proposes RLTrajGen-PPMPC-CBF, a hierarchical framework for safe, smooth and comfort roundabout navigation, which regulates the coupling between RL-based planning and MPC-based control. We employ Prescribed Performance Constraints (PPC) to enforce a gradual, stable convergence between reference trajectories and control outputs, ensuring MPC tracking performance remains consistent with intended behavior from RL. Additionally, a Control Barrier Function (CBF) layer provides real-time safety corrections that are fed back into the RL process. Simulation results in the MetaDrive environment demonstrate that our method achieves a 6.25\% increase in average success rate and a 65.87\% reduction in Motion Sickness Dose Value (MSDV) compared to the optimal baseline, meanwhile accelerating training convergence.

==> sections/conclusion.tex <==
%By introducing a Trajectory Generator and the PPC mechanism into the RL-MPC-CBF framework, this study not only improves the performance of reinforcement learning, but also directly addresses the oscillation problem of the agent caused by the structural mismatch between RL and MPC. Furthermore, owing to the property of progressive convergence, the decision-making process of the autonomous driving algorithm becomes smoother and more gradual, significantly reducing the MSDV value. 

%Four baseline methods are constructed and compared in a modular manner to analyze the contribution of each component. Finally, experiments are conducted on the MetaDrive simulation platform, and the results demonstrate the superiority of the proposed algorithm.

%This study presents a new-designed Trajectory Generator module and a PPC mechanism within the RL-MPC hierarchical framework, significantly accelerating the convergence of RL training and improving the trajectory planning performance in autonomous driving contexts. 

This work proposes a hierarchical learning based control framework for roundabout navigation of CAVs. By addressing the oscillation issues caused by the structural mismatch between RL and MPC, our approach facilitates smoother and more gradual decision-making processes. Meanwhile, the safety criteria are ensured by a CBF layer, which also allows the agent to learn the revised actions. Experiments on the MetaDrive simulation platform validate the superior performance of our proposed algorithm through the construction and modular comparison of five baseline methods. Our framework not only achieves the highest average reward and success rate, but also generates the smoothest trajectory measured by MSDV and JERK, demonstrating its potential for real-world applications in complex driving scenarios. Future works will extend this framework to enhance navigation robustness in more complex environments.

==> sections/experiment.tex <==
\subsection{Simulation Platform Setup}
The roundabout simulation environment built in MetaDrive is shown in \Figref{fig:metadrive-env}, with some key parameters listed.
%MetaDrive has a built-in roundabout map, as shown in \Figref{fig:metadrive-env}, some key parameters have also been listed. 
%the desired distance between a vehicle and its preceding vehicle. 
The computer used for reinforcement learning is equipped with an AMD EPYC 7453 processor, with CUDA version 12.9 and Python version 3.11.4. During training, four parallel environments are used for sampling, followed by training on an NVIDIA RTX 4090 GPU. A fixed random seed is set at the initialization of each process to ensure the reproducibility of the experiments. The key hyperparameters of the framework listed in \Figref{fig:metadrive-env} have been manually carefully tuned.

\begin{figure}[tp]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/check.pdf}
    \caption{(\textbf{left}) Simulation environment diagram. (\textbf{right}) Training Hyperparameter Table.}
    \vspace{-15pt}
    \label{fig:metadrive-env}
\end{figure}

\subsection{Benchmark Comparison}

\begin{table}[tp]
    \centering
    \tablecaption{Methods Overview}
    \input{tabs/tab5.tex}
    \vspace{-15pt}
    \label{tab:methods}
\end{table}

We select three baselines as the main comparison methods, namely PPO-only, PPO-MPC, and CBFG-PPO from~\cite{zhangControlBarrierFunctionGuided2025}. Detailed descriptions of these methods are provided in \Tabref{tab:methods}. During training, a monitor is employed to record the average reward(AR) and average success rate(ASR) of each episode. The collected data are smoothed using a sliding window and are illustrated in \Figref{fig:avg-reward} and \Figref{fig:success-rate}. As shown in these figures, \Medref{M6} achieves the highest AR and ASR, reaching 178.05 and 96.25\%, respectively. These results outperform PPO-only (AR 156.74, ASR 67.50\%), PPO-MPC (AR 159.18, ASR 63.75\%), and CBFG-PPO (AR 161.59, ASR 77.50\%). Otherwise, among all compared methods, \Medref{M6} exhibits the fastest convergence. Specifically, it converges within approximately 1300 steps, whereas the other baseline methods typically require about 3000--5000 steps to reach convergence.

The optimal policy from each method is implemented in the ego vehicle and assessed in the simulation environment. \Figref{fig:phsical-state} illustrates the changes in velocity, heading angle, acceleration, and steering angle during driving, while \Figref{fig:position} displays the actual driven trajectory. Compared to the baselines, our method keeps acceleration and steering angle within a narrower range, ensuring smoother and safer vehicle behavior. Additionally, our approach employs a distinct route planning strategy by selecting lanes with fewer surrounding vehicles and executing gradual lane changes at lower speeds, thereby enhancing ride comfort in autonomous scenarios.
%The optimal policy obtained by each method is then deployed on the ego vehicle and evaluated in the simulation environment. The variations of velocity, heading angle, acceleration, and steering angle during driving are illustrated in \Figref{fig:phsical-state}, while the actual driven trajectory is shown in \Figref{fig:position}. From these results, it can be observed that, compared with the baselines, our method maintains acceleration and steering angle within a relatively small range throughout the driving process, leading to smoother and safer vehicle behavior. Moreover, our method adopts a different route planning strategy from the baselines by proactively selecting lanes with fewer surrounding vehicles and performing gradual lane changes at reduced speed, which significantly improves ride comfort in autonomous driving scenarios.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/new_version/avg_reward.pdf}
    \caption{ AR evolution curves of all methods during training. }
    \vspace{-5pt}
    \label{fig:avg-reward}
    \vspace{-5pt}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/new_version/success_rate.pdf}
    \caption{ ASR evolution curves of all methods during training. }
    \vspace{-15pt}
    \label{fig:success-rate}
    \vspace{-5pt}
\end{figure}

\subsection{Ride comfort and behavior} \label{md:comfort}
To evaluate the comfort of algorithms during driving, appropriate metrics must be selected. Following the ISO 2631 standard, the weighted root-mean-square (RMS) of each acceleration component is commonly used to measure vehicle roughness~\cite{aledhariMotionComfortOptimizationforAutonomous2024}. Accordingly, the motion sickness dose value (MSDV) is adopted as an indicator of motion sickness and is defined as:
\begin{equation}
\mathrm{MSDV} = \sqrt{\int_0^T [\tilde{a}(t)]^2 \,\mathrm{d}t}
\end{equation}
where $T$ denotes the observation duration, and $\tilde{a}(t)$ represents the weighted acceleration (including both longitudinal and lateral components). Considering both longitudinal and lateral accelerations, the discrete forms of MSDV are expressed as:
\begin{equation}
\mathrm{MSDV}_V = \sqrt{\frac{1}{N}\sum_{i=1}^N a_{x,i}^2},\, \mathrm{MSDV}_L = \sqrt{\frac{1}{N}\sum_{i=1}^N a_{y,i}^2}
\end{equation}
where $a_{x,i}$ is the longitudinal acceleration at time step $i$, directly obtained from the simulation. $a_{y,i}$ is the lateral acceleration at time step $i$, estimated by $a_{y,i} = (\delta_{i+1} - \delta_i)v_i / \Delta t$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=17.5cm,height=7.2cm]{figs/new_version/physical_state.pdf}
    \caption{ Velocity, heading angle, acceleration, and steering angle profiles compared with baselines and ablation studies. }
    \vspace{-5pt}
    \label{fig:phsical-state}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=8.5cm,height=3.5cm]{figs/new_version/position.pdf}
    \caption{Visualized real-time motion trajectories under different approaches.}
    %\vspace{-15pt}
    \label{fig:position}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=8.5cm,height=7.2cm]{figs/new_version/msdv_jerk.pdf}
    \caption{Comparison of $\mathrm{MSDV}$ and $\mathrm{JERK}$.}
    \vspace{-15pt}
    \label{fig:msdv-jerk-bar}
\end{figure}

\begin{table}[tp]
    \centering
    \tablecaption{Indicator Comparison}
    \resizebox{\linewidth}{!}{%
        \input{tabs/tab6.tex}
    }
    \vspace{-15pt}
    \label{tab:indicator-comparison}
\end{table}

In addition to MSDV, human perception is particularly sensitive to changes in acceleration, motivating the use of JERK as another comfort metric, defined as:
\begin{equation}
\mathrm{JERK} = \sqrt{\int_0^T \left[\frac{\mathrm{d}a}{\mathrm{d}t}\right]^2 \mathrm{d}t}
\end{equation}
Its discrete longitudinal and lateral forms are given by:
\begin{equation}
\mathrm{JERK}_V = \sqrt{\sum_{i=1}^N \mathrm{diff}(a_{x,i})^2},\, \mathrm{JERK}_L = \sqrt{\sum_{i=1}^N \mathrm{diff}(a_{y,i})^2}
\end{equation}

All methods in \Tabref{tab:methods} are evaluated using the MSDV and JERK metrics, and the corresponding results are illustrated in \Figref{fig:msdv-jerk-bar}. \Medref{M6} achieves the lowest values in $\mathrm{MSDV}_V$ (0.457), $\mathrm{MSDV}_L$ (0.449), and $\mathrm{JERK}_L$ (8.815). Although its $\mathrm{JERK}_V$ value (2.483) is slightly higher than that of \Medref{M1} (1.714) and \Medref{M5} (2.229), the proposed method overall demonstrates the best ride comfort among all evaluated approaches.

\subsection{Ablation Study and Analysis}
To validate the effectiveness of RLTrajGen and PPMPC, we conducted two ablation experiments: RLTrajGen-MPC-CBF and RL-PPMPC-CBF. These experiments are designed to explore the individual contributions of each module. Detailed descriptions of the methods can be found in \Tabref{tab:methods}.

%To assess the effectiveness of RLTrajGen and PPMPC, we conducted two ablation experiments: RLTrajGen-MPC-CBF and RL-PPMPC-CBF. These experiments are designed to explore the individual contributions of each module. Detailed descriptions of the methods can be found in \Tabref{tab:methods}.
\vspace{+5pt}

\noindent\textbf{Effect of the RLTrajGen module.} 
The replacement of the RL module in \Medref{M3} with the RLTrajGen module results in \Medref{M4}. In terms of AR, \Medref{M4} demonstrates faster convergence compared to \Medref{M3}, indicating that RLTrajGen significantly enhances convergence speed. However, the overall performance of \Medref{M4} is notably inferior to that of other benchmarks, suggesting that merely incorporating RLTrajGen is not sufficient for optimal results. In addition, \Medref{M5} removes the RLTrajGen module from the complete framework \Medref{M6}. The experimental results show that \Medref{M6} achieves faster convergence in both AR and ASR than \Medref{M5}. These findings indicate that the Trajectory Generator resolves the structural mismatch between RL and MPC which accelerated the agent's learning process.
%Replacing the RL module in \Medref{M3} with the RLTrajGen module yields \Medref{M4}. In terms of AR and ASR, both \Medref{M4} and \Medref{M6} exhibit faster convergence than the other methods, indicating that RLTrajGen can significantly accelerate convergence. However, the overall performance of \Medref{M4} is notably worse than that of the other benchmarks. This degradation may be attributed to the fact that, after the RL module outputs a trajectory, the MPC tends to place insufficient emphasis on the cost induced by trajectory tracking errors, and instead prioritizes reducing control effort. Consequently, the overall performance gradually deteriorates. This observation also suggests that constraining trajectory tracking errors with fixed weights is generally impractical: if the weight is set too small, MPC may ignore trajectory errors, whereas if it is set too large, the optimization problem may become infeasible. Therefore, a cost function that progressively enforces trajectory accuracy over time, as adopted in the proposed PPMPC, is necessary.

%Comparing \Medref{M5} and \Medref{M6}, since \Medref{M5} does not incorporate the RLTrajGen module, MPC employs PPC as the cost function while solving a target-enclosing task. The inherent lack of structural coupling still results in larger oscillations in acceleration and steering angle compared with \Medref{M6}, leading to lower AR and success rate. These results clearly demonstrate that, when combined with PPMPC, the RLTrajGen module enables smoother and safer vehicle motion.


\noindent\textbf{Effect of the PPMPC module.} 
\Medref{M5} is obtained by replacing the MPC module in \Medref{M3} with PPMPC. This leads to a substantial change in vehicle behavior: the overall profiles of velocity, heading angle, acceleration, and steering angle reduce to fewer oscillations, resulting in a smoother trajectory in \Figref{fig:position}. This improvement arises because traditional MPC often neglects the cost induced by trajectory tracking errors, focusing instead on reducing control effort, which can gradually deteriorate performance. Meanwhile, constraining trajectory tracking errors with fixed weights is generally impractical: if the weight is set too small, MPC may ignore trajectory errors, whereas if it is set too large, the optimization problem may become infeasible. Therefore, the PPMPC module needs to be integrated with RL for more flexible parameters. By comparing the average success rate of \Medref{M5} and \Medref{M3}, PPMPC substantially improves safety, increasing the success rate from 77.50\% to 96.25\%. In addition, PPMPC achieves markedly better performance in terms of MSDV and JERK than \Medref{M3}, further demonstrating enhanced ride comfort.

%This degradation may be attributed to the fact that, after the RL module outputs a trajectory, the MPC tends to place insufficient emphasis on the cost induced by trajectory tracking errors, and instead prioritizes reducing control effort. Consequently, the overall performance gradually deteriorates. This observation also suggests that constraining trajectory tracking errors with fixed weights is generally impractical: if the weight is set too small, MPC may ignore trajectory errors, whereas if it is set too large, the optimization problem may become infeasible. Therefore, a cost function that progressively enforces trajectory accuracy over time, as adopted in the proposed PPMPC, is necessary.

%Furthermore, as discussed in the analysis of the RLTrajGen module, PPMPC provides a significant performance improvement when only the RLTrajGen module is included. Both driving behavior and quantitative metrics, including AR and ASR, are improved from suboptimal levels to the best performance among all methods.



==> sections/introduction.tex <==
The advancement of Intelligent Transportation Systems (ITS) has accelerated the deployment of Connected and Autonomous Vehicles (CAVs), enabling them to navigate diverse urban environments~\cite{ahmedTechnologyDevelopmentsImpacts2022,ranaConnectedAutonomousVehicles2023}. Significant progress has been achieved in standard driving tasks, including lane keeping~\cite{dingAdaptiveMemoryEventTriggered2024,pachpolEnhancedLaneKeeping2024,dingIntelligentEventTriggered2025}, lane changing~\cite{zhangControlBarrierFunctionGuided2025,wangResearchAutonomousDriving2024}, and adaptive cruise control~\cite{heAdaptiveCruiseControl2019,xiaoComprehensiveReviewDevelopment2010}. However, roundabouts remain particularly challenging due to dense vehicle interactions and rapidly changing traffic conditions, where planning or control failures may compromise both safety and ride comfort~\cite{dingAdaptiveMemoryEventTriggered2024,nakayaExplorationDeepReinforcement2025}.

Current autonomous driving approaches mainly fall into learning-based and model-based methods. Reinforcement Learning (RL) has demonstrated strong capability in high-dimensional perception and decision-making~\cite{antonioMultiAgentDeepReinforcement2022,zhouDevelopmentEfficientDriving2020,liuCuriositydrivenReinforcementLearning2025,huCoMoCAVsCohesiveDecisionGuided2025a}. However, its model-free nature makes it difficult to explicitly incorporate vehicle dynamics and safety constraints~\cite{brunkeSafeLearningRobotics2022,wuRecentAdvancesReinforcement2024}. In contrast, Model Predictive Control (MPC) explicitly considers system dynamics and constraints, while Control Barrier Functions (CBFs) have been widely integrated into MPC to provide formal safety guarantees~\cite{seoSafetyCriticalControlNonaffine2022,xiaoSafeAutonomyControl2023,amesControlBarrierFunctions2019}. Nevertheless, model-based approaches generally exhibit limited adaptability in highly dynamic environments.


\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/fig2-2.pdf}
    \caption{ Comparison between the proposed method (\textbf{bottom left}) and baseline approaches (\textbf{upper left}). We constrain the errors between RL and MPC outputs in prescribed performance bounds to improve trajectory planning performance. }
    \vspace{-15pt}
    \label{fig:roundabout}
\end{figure}

To combine the adaptability of RL with the safety and constraint-handling capability of MPC, hybrid RL-MPC frameworks have attracted increasing attention~\cite{reiterSynthesisModelPredictive2025a,zhouEnhancePlanningPhysicsinformed2024,oliveiradasilvaIntegratingReinforcementLearning2025a,lubarsCombiningReinforcementLearning2021}. Oliveira et al.~\cite{oliveiradasilvaIntegratingReinforcementLearning2025a} employed RL to determine discrete decision variables for accelerating MPC optimization, while Lubars et al.~\cite{lubarsCombiningReinforcementLearning2021} combined DDPG with MPC, where MPC served as a safety fallback for potentially unsafe RL actions. Zhang et al.~\cite{zhangControlBarrierFunctionGuided2025} further incorporated a CBF safety filter into an RL-MPC framework (\Figref{fig:roundabout}(b)). Nevertheless, these methods still suffer from a structural mismatch: RL produces pointwise decisions whereas MPC optimizes trajectories, limiting MPC's ability to accurately realize the planning intent and resulting in less smooth trajectories in complex driving scenarios.
Zhang et al.~\cite{zhangControlBarrierFunctionGuided2025} introduced a CBFG-PPO framework (\Figref{fig:roundabout} (b)), where RL provides target states for MPC, and CBF filters unsafe actions and feeds corrections back to RL.
Nevertheless, RL produces pointwise decisions while MPC optimizes over trajectories in this framework, which results in structural mismatch and limits MPC’s ability to accurately realize RL intent, producing less smooth trajectories for CAVs in complex environments.

 
 %\textcolor{blue}{To address this mismatch, we first introduce a trajectory generator that transforms the pointwise outputs of RL into reference trajectories for MPC tracking. Furthermore, we incorporate a prescribed performance constraint (PPC) mechanism to progressively reduce the tracking error, enabling MPC to more accurately follow the trajectories generated by RL. This design improves the consistency between planning and control, facilitating more stable policy learning and enhanced navigation performance.}

To address the mentioned issues, we propose a novel RLTrajGen-PPMPC-CBF framework, as illustrated in \Figref{fig:roundabout} (c), and validate its effectiveness in a roundabout scenario. The proposed framework consists of three key components: an RL-based Trajectory Generator (RLTrajGen) that facilitates high-level decision making by producing reference trajectories, a prescribed performance MPC (PPMPC) that dynamically adjusts trajectory tracking within a predefined performance envelope, and a CBF-based safety filter that corrects unsafe behaviors. Specifically, we first introduce a trajectory generator that transforms the pointwise outputs of RL into reference trajectories for MPC tracking. Furthermore, we incorporate a prescribed performance constraint (PPC) mechanism to progressively reduce the tracking error, enabling MPC to more accurately follow the trajectories generated by RL. This design improves the consistency between planning and control, facilitating more stable policy learning and enhanced navigation performance. The main contributions of this work are summarized as follows:

\begin{enumerate}
    \item We design a trajectory generation mechanism that converts single-step outputs from RL into trajectories with adaptive parameters for MPC tracking, thereby effectively resolving the structural mismatch between RL and MPC and significantly accelerating the convergence speed of training.
    \item We utilize PPC to regulate the coupling between RL-based planning and MPC-based control, which is the first one in RL-MPC hierarchical framework to our best knowledge. Our method facilitates the progressive reduction of trajectory tracking errors between the planning and control layers, thus balancing the adaptability to complex scenarios and the safety for autonomous systems, and improving ride comfort by producing smoother trajectories.
\end{enumerate}

%The remainder of this paper is organized as follows. \Secref{sec:preliminaries} introduces the problem formulation. \Secref{sec:method} presents the proposed RLTrajGen-PPMPC-CBF framework. \Secref{sec:experiments} includes simulation results. \Secref{sec:conclusion} concludes the paper.



==> sections/method.tex <==
\subsection{Framework Overview}\label{med:overview}
The proposed framework consists of three coupled layers, as illustrated in \Figref{fig:framework}: 
1) a high-level decision-making layer that specifies reference motion intentions through a learned policy; 
2) a low-level control layer that tracks the resulting reference trajectory and computes control inputs based on the dynamic model; and 
3) a safety mediation layer that corrects unsafe behaviors during execution.

In general, the framework follows a standard reinforcement learning training and evaluation pipeline. 
At each time step, the high-level agent produces actions that generate a reference state sequence $\bm{z}^*_t$ of length $n_p$:
\begin{equation}
    \bm{z}^*_t = \{\bm{z}^*_{t+i}\} = \{(v^*_{t+i}, \theta^*_{t+i}) \mid i=0,1,\cdots,n_p-1\}
    \label{eq:state-sequence}
\end{equation}
where $\bm{z}^*_t$ represents the desired future motion of the ego vehicle. 
The low-level controller is responsible for tracking this reference trajectory, and the corresponding tracking error $e$ incorporated into the cost function MPC is given as:
\begin{equation}
    e = \mathrm{dist}(\bm{z}_t, \bm{z}^*_t)
    \label{eq:mpc-rl-error}
\end{equation}
where $\bm{z}_t$ denotes the trajectory generated by MPC and $\mathrm{dist}(\cdot)$ measures the deviation from the reference. 
%After potential unsafe action output by MPC is corrected by a CBF-based filter, the resulting control input $\bm{u}_t = [a_t, \delta_t]^T$ is applied to the simulated vehicle, which interacts with the environment and returns a reward, thereby completing one training iteration.
After any potentially unsafe action output from the MPC is corrected using a CBF-based filter, the resulting control input $\bm{u}_t = [a_t, \delta_t]^T$ is applied to the simulated vehicle. This interaction with the environment yields a reward, thereby completing one training iteration.

\begin{table}[tp]
    \centering
    \tablecaption{Rewards Composition}
    \input{tabs/tab2.tex}
    \vspace{-15pt}
    \label{tab:rewards}
\end{table}

\subsection{RL-based Trajectory Generator}\label{med:rl}
The surrounding environment is perceived through onboard sensors, such as LiDAR, and encoded into a $259$-dimensional observation vector. This vector contains various parameters including the vehicle speed $v_t$, steering angle $\delta_t$, previous throttle/brake command $u_{t-1}$, previous steering angle $\delta_{t-1}$, yaw rate $r_t$, heading difference to the lane $\Delta \psi$, distances to the left and right lane boundaries $d_L$ and $d_R$, lateral lane position $p_{lat}$, projected distances along the lane heading $d_{\parallel}$, projected lateral distances $d_{\perp}$, lane curvature radius $R$, turn direction flags $C$, lane angles $\theta$, and surrounding LiDAR features $\bm{s}^{sur}_t$.

%The action space is four-dimensional and jointly parameterizes a reference trajectory and its tracking weights. Specifically, the action is defined as $\bm{a}_t = (\bm{q}_t, \bm{w}_t)$, where $\bm{q}_t = [\nu_t^*, \kappa_t^*] \in \mathbb{R}^2$ specifies the structure of a Trajectory Generator $\mathcal{G}_t(\bm{x}_t;\bm{q}_t):\mathbb{R}^4\to\mathbb{R}^{2\times n_p}$ and thereby determines the reference trajectory, while $\bm{w}_t = [w_t^v, w_t^\theta] \in \mathbb{R}^2$ is a weight vector that adjusts the strictness of trajectory tracking in the MPC.  Once $\bm{q}_t$ is specified, the form of the Trajectory Generator $\mathcal{G}_t$ is fixed, and the resulting reference trajectory $\bm{z}_t^*$ is generated according to
The action space includes adjustable parameters for a generated reference trajectory and its prescribed performance tracking weights. Specifically, the action is defined as $\bm{a}_t = (\bm{q}_t, \bm{w}_t)$. 
$\bm{w}_t = [w_t^v, w_t^\theta] \in \mathbb{R}^2$ is a weight vector that adjusts the strictness of the prescribed  trajectory tracking performance in the MPC.
$\bm{q}_t = [\nu_t^*, \kappa_t^*] \in \mathbb{R}^2$ specifies the structure of a Trajectory Generator $\mathcal{G}_t(\bm{x}_t;\bm{q}_t):\mathbb{R}^4\to\mathbb{R}^{2\times n_p}$ and helps to generate the reference trajectory by the following state transition function:
\begin{equation}
    \left\{
    \begin{array}{l}
    v_{t+i}^* = \nu_t^*, \, i=0,\cdots,n_p-1, \\
    \theta_{t+i}^* = \theta_{t+i-1}^* + v_{t+i-1}^*\kappa_t^*\Delta t, \, i=1,\cdots,n_p-1, \\
    \theta_t^* = \theta_t.
    \end{array}
    \right.
    \label{eq:traj-generator}
\end{equation}
\Figref{fig:traj-ppc} illustrates a segment of the resulting reference trajectory. The velocity profile is piecewise constant, while the heading angle evolves as a continuous piecewise linear function. By modifying the Trajectory Generator, different reference trajectory shapes can be obtained.

Based on the optimal control problem defined in \eqref{final-problem}, two reward terms are designed: $r_1$ for goal-reaching behavior and $r_2$ for collision avoidance, which are presented in \Tabref{tab:rewards} in detail. 
Specifically, $r_1$ is composed of four components as $r_1 = r_{\mathrm{dest}} + r_{\mathrm{speed}} + r_{\mathrm{steer}} + r_{\mathrm{terminal}}$. Here, $r_{\mathrm{dest}} = \Vert \bm{l}_t - \bm{l}_{t-1} \Vert$ measures progress toward the goal, $r_{\mathrm{speed}} = v_t / v_{\max}$ encourages efficient motion, $r_{\mathrm{steer}} = -\Vert \theta_t - \theta_{t-1} \Vert$ penalizes abrupt steering changes, and $r_{\mathrm{terminal}} = 10$ is assigned upon successful arrival. 
Meanwhile, the collision-related reward is defined as $r_2 = r_{\mathrm{crash}}$, where $r_{\mathrm{crash}} = -5$ in the event of a collision and $0$ otherwise.


\begin{figure}[tp]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/fig4-5.pdf}
    \caption{(\textbf{left}) Discrete-time performance verification for five cases: continuous-time baseline, constant weight($\mathrm{e}^{-\iota\Delta t}$), and random weights from normal distributions $\mathcal{N}\sim(\mathrm{e}^{-\iota\Delta t}, \sigma^2)$ where $\sigma=0.1/0.2/0.3$. (\textbf{right}) Schematic of the reference Trajectory Generator parameterized by $(\nu_t^*, \kappa_t^*)$.}
    \vspace{-5pt}
    \label{fig:traj-ppc}
\end{figure}

\begin{figure}[tp]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/fig6.pdf}
    \caption{The establishment of collision avoidance diagrams.}
    \vspace{-15pt}
    \label{fig:cbf-dem}
\end{figure}

Proximal Policy Optimization (PPO) is adopted for policy learning. 
The policy network $\pi_\theta(\bm{a}_t|\bm{o}_t)$ generates actions from observations, while the value network $V_\omega(\bm{o}_t)$ estimates the state value. 
The Generalized Advantage Estimation (GAE) is computed as
\begin{equation}
    \hat{A}_t = \delta_t + \gamma\lambda(1-d_{t+1})\hat{A}_{t+1},
    \label{eq:gae-formulation}
\end{equation}
\begin{equation}
    \delta_t = r_t + \gamma(1 - d_{t+1})V_{t+1} - V_t
    \label{eq:caculate-delta}
\end{equation}
where $V_t = V_\omega(\bm{o}_t)$ represents the value function, $r_t$ denotes the reward, $d_t$ indicates episode termination, $\gamma$ is the discount factor, and $\lambda$ controls the bias--variance trade-off.

The loss functions of the two networks in PPO are given by:
\begin{equation}
    L^{\mathrm{CLIP}}(\theta) = \hat{\mathbb{E}}_t[\min(r_t(\theta)\hat{A}_t, \mathrm{clip}(r_t(\theta), 1-\varepsilon, 1+\varepsilon)\hat{A}_t)],
    \label{eq:policy-loss-function}
\end{equation}
\begin{equation}
    L(\omega) = \hat{\mathbb{E}}_t[(r_t + \gamma V_\omega(\bm{o}_{t+1}) - V_\omega(\bm{o}_t))^2]
    \label{eq:value-loss-function}
\end{equation}
where $\mathrm{clip}$ is a clipping function that constrains $r_t(\theta)$ to $[1-\varepsilon, 1+\varepsilon]$, and $r_t(\theta) := \pi_\theta(\bm{a}_t|\bm{o}_t) / \pi_{\theta_{\mathrm{old}}}(\bm{a}_t|\bm{o}_t) $. The final training objective is a weighted combination of the policy and value losses:
\begin{equation}
    L_{\mathrm{final}} = a_1 L^{\mathrm{CLIP}}(\theta) + a_2 L(\omega),\, a_i \in (0,1),\, i=1,2.
    \label{eq:loss-final}
\end{equation}

\subsection{MPC with PPC-based cost}\label{med:mpc-ppc}
PPC progressively shrinks the error bounds, ensuring that the error asymptotically converges to a specified value. This characteristic can be directly integrated into the construction of $ \mathrm{dist}(\bm{z}_t, \bm{z}^*_t)$ in \eqref{eq:mpc-rl-error}. Given that $ \mathrm{dist}(\bm{z}_t, \bm{z}^*_t)$ is evaluated in discrete time, the performance function in PPC must first be discretized.
Denoting the sampling interval as $\Delta t$ and defining a discrete-time performance function $p_k = p(k\Delta t)$, we obtain:
\begin{equation}
    p_{k+1} = p((k+1)\Delta t) = w p_k + (1 - w)p_{\infty}
    \label{eq:dicrete-time-equation-derivation}
\end{equation}
Following \cite{buDiscreteTimePrescribedPerformance2023, liuPrescribedPerformanceModelFree2019}, 
the parameter $w = \exp(-\iota\Delta t)$ is treated as time-varying, i.e., $w=w_k:=w(k)$. Then, \eqref{eq:dicrete-time-equation-derivation} can be rewritten as:
\begin{equation}
    p_{k+1} = w_k p_k + (1 - w_k)p_{\infty},\, k=0,1,\dots,+\infty
    \label{eq:dicrete-time-equation-derivation-final}
\end{equation}
The effectiveness of \eqref{eq:dicrete-time-equation-derivation-final} can be verified in \Figref{fig:traj-ppc}. The error transformed by this discrete-time performance metric is used to define the distance function:
\begin{equation}
    \begin{aligned}
    \mathrm{dist}(\bm{z}_t, \bm{z}_t^*) 
    &= \mathrm{dist}([v_t,\theta_t],[v_t^*,\theta_t^*]) \\
    &= \left\Vert\big[\Xi^{-1}(\bar{e}_t^v), \Xi^{-1}(\bar{e}_t^\theta)\big]\right\Vert
    \end{aligned}
    \label{eq:dist-definetion}
\end{equation}
where the normalized errors $\bar{e}_t^v$, $\bar{e}_t^\theta$ are defined as
\begin{equation}
    \bar{e}_t^v = \frac{v_t - v_t^*}{p_\tau^v}, \,
    \bar{e}_t^\theta = \frac{\theta_t - \theta_t^*}{p_\tau^\theta}.
    \label{eq:barerror-explanation}
\end{equation}
Here, $p_\tau^v$ and $p_\tau^\theta$ are the discrete-time performance functions for $v$ and $\theta$, respectively. The two performance functions correspond to weights $\bm{w}_t = [w_t^v, w_t^\theta] \in \mathbb{R}^2$ introduced in \Secref{med:rl}.
The PPC timer is reset at the beginning of each episode, and $\tau$ denotes the relative time within the episode. 
%Since two performance functions are employed, two corresponding weights are required, which explains why $\bm{w}\in\mathbb{R}^2$ as introduced in \Secref{med:rl}.

With the defined PPC-based distance function, the MPC problem is then formulated as
\begin{equation}
    \begin{aligned}
    &\underset{\bm{u}}{\min}\; J(\bm{z}_t^{t+n_p},\bm{u}_t^{t+n_p-1}) = \\
    &\sum_{i=0}^{n_p-1}
    \left[
    \underbrace{\mathrm{dist}(\bm{z}_{t+i}, \bm{z}_{t+i}^*)}_{\text{state error}}
    +
    \underbrace{\Vert \bm{u}_{t+i}\Vert}_{\text{control cost}}
    \right]
    +
    \underbrace{\mathrm{dist}(\bm{z}_{t+n_p}, \bm{z}_{t+n_p}^*)}_{\text{terminal cost}} \\
    &s.t.
    \left\{\begin{array}{l}
    \bm{x}_{t+i+1} = \hat{f}(\bm{x}_{t+i}, \bm{u}_{t+i}), \\
    \bm{z}_{t+i} = [\bm{0}_{2\times 2}, \bm{I}_{2\times 2}] \bm{x}_{t+i}, \\
    \bm{u}_{\min} \le \bm{u}_{t+i} \le \bm{u}_{\max}, \, i=0,\dots,n_p-1
    \end{array}\right.
    \end{aligned}
    \label{eq:mpc-formulation}
\end{equation}
where $\bm{0}_{2\times 2}$ and $\bm{I}_{2\times 2}$ denote the zero and identity matrices, respectively, and $\hat{f}$ follows the dynamics in \eqref{eq:discrete-dynamic-evaluate-eq}. 
Solving \eqref{eq:mpc-formulation} yields the optimal state and control sequences. 
We define $\bm{x}_t^{\mathrm{MPC}} = \bm{x}_{t+1}$, 
$\bm{z}_t^{\mathrm{MPC}} = [\bm{0}_{2\times 2}, \bm{I}_{2\times 2}] \bm{x}_t^{\mathrm{MPC}}$, 
and denote the applied control as $\bm{u}_t^{\mathrm{MPC}}$, 
which will be used in \Secref{med:cbf}.

\subsection{CBF-based safety filter}\label{med:cbf}
CBF is employed to synthesize a safety filter to correct potentially unsafe behaviors generated by MPC. 
In a roundabout scenario, the primary safety objective is to avoid inter-vehicle collisions. 
To this end, each vehicle is approximated by an ellipse, which enables a quantitative formulation of collision-avoidance constraints. 
As illustrated in \Figref{fig:cbf-dem}, a vehicle is first approximated by a rectangle and then enclosed by a circumscribed ellipse. 
Let $a$ and $b$ denote the semi-major and semi-minor axes, respectively. 
The equation of a non-rotated ellipse centered at $\bm{x}_o$ is $(\bm{x}-\bm{x}_o)^T \bm{D} (\bm{x}-\bm{x}_o)=1$, where $\bm{D}=\mathrm{diag}(1/a^2,\,1/b^2)$.

For an ellipse rotated by an angle $\theta$, a coordinate transformation is applied using the rotation matrix $\bm{R}_\theta=[\cos\theta,\sin\theta;-\sin\theta,\cos\theta]$, yielding
$(\bm{x}-\bm{x}_o)^T \bm{R}_\theta^T \bm{D} \bm{R}_\theta (\bm{x}-\bm{x}_o)=1$.
Then, let $\bm{Q}_\theta=\bm{R}_\theta^T \bm{D}\bm{R}_\theta$. 
To compute the distance between two ellipses, consider the line connecting their centers, along which a point is given by $\bm{x}=\bm{x}_o+\bm{e}t$, where $\bm{e}$ is the unit direction vector. 
Substituting into the ellipse equation yields $t=1/\sqrt{\bm{e}^T\bm{Q}_\theta\bm{e}}$. 
Accordingly, the distance between the boundaries of two ellipses is defined as
$d_{\mathrm{F}}(\bm{x})=\Vert \bm{e}_{o_{1,2}}\Vert-1/\sqrt{\bm{e}^T\bm{Q}_\theta\bm{e}}-1/\sqrt{\bm{e}^T\bm{Q}_\varphi\bm{e}}$,
where $\bm{e}_{o_{1,2}}=\bm{x}_{o_1}-\bm{x}_{o_2}$ and $\bm{e}=\bm{e}_{o_{1,2}}/\Vert \bm{e}_{o_{1,2}}\Vert$. 
The obstacle-avoidance function is then defined as $h(\bm{x}) = d_{\mathrm{F}}(\bm{x}) - d_{\min}$. 
For clarity, only one safety constraint is considered here. 
The resulting CBF optimization problem is formulated as:
\begin{equation}
    \begin{aligned}
    &\underset{\bm{u}}{\min}\, J(\bm{u}_t) = \Vert \bm{u}_t - \bm{u}_t^{\mathrm{MPC}}\Vert \\
    &s.t.\left\{\begin{array}{l}
    \bm{x}_{t+1} = \hat{f}(\bm{x}_t, \bm{u}_t),  \\
    h(\bm{x}_{t+1}) - (1 - \gamma)h(\bm{x}_t) \ge 0.
    \end{array}\right.
    \end{aligned}
    \label{eq:cbf-formulation}
\end{equation}
Solving \eqref{eq:cbf-formulation} yields $\bm{x}_{t+1}$ and $\bm{u}_t$, which are denoted as $\bm{x}_t^{\mathrm{CBF}} = \bm{x}_{t+1}$ and $\bm{u}_t^{\mathrm{CBF}} = \bm{u}_t$. 
The corresponding state representation is defined as $\bm{z}_t^{\mathrm{CBF}} = [\bm{0}_{2\times2}, \bm{I}_{2\times2}] \bm{x}_t^{\mathrm{CBF}}$.

Inspired by \cite{zhangControlBarrierFunctionGuided2025}, the policy loss in \eqref{eq:policy-loss-function} is modified to enable the reinforcement learning agent to learn CBF-induced corrective behavior:
\begin{equation}
    \begin{aligned}
    &L^{\mathrm{CLIP}}(\theta) = \\
    &\left\{\begin{array}{l}
    \mathbf{case\;1}\; \Vert\bm{z}_t^{\mathrm{CBF}}-\bm{z}_t^{\mathrm{MPC}}\Vert<\delta_{\bm{z}} \\
    \hat{\mathbb{E}}_t[\min(r_t(\theta)\hat{A}_t, \mathrm{clip}(r_t(\theta), 1-\varepsilon, 1+\varepsilon)\hat{A}_t)],\\
    \\
    \mathbf{case\;2}\; \Vert\bm{z}_t^{\mathrm{CBF}}-\bm{z}_t^{\mathrm{MPC}}\Vert \ge\delta_{\bm{z}} \\
    \hat{\mathbb{E}}_t[\bm{z}_t^{\mathrm{CBF}}-[\bm{I}_{2\times2},\bm{0}_{2\times1}]\bm{\mu}_t(\theta)].
    \end{array}\right.
    \end{aligned}
    \label{eq:policy-loss-function-modify}
\end{equation}
In \eqref{eq:policy-loss-function-modify}, $\delta_{\bm{z}}$ denotes the threshold beyond which CBF intervention is considered significant. 
If so, the original loss is replaced by \textbf{case 2}, encouraging the policy mean $\bm{\mu}_t(\theta)= \mathbb{E}_{\bm{a}_t\sim \pi_\theta(\bm{a}_t|\bm{o}_t)}[\bm{a}_t] \in \mathbb{R}^4$ to align with the CBF-corrected state.
%\begin{equation}
    %\bm{\mu}_t(\theta) = \mathbb{E}_{\bm{a}_t\sim \pi_\theta(\bm{a}_t|\bm{o}_t)}[\bm{a}_t] \in \mathbb{R}^4
    %\label{eq:policy-mean}
%\end{equation} 

==> sections/preliminaries.tex <==
\subsection{System Model} \label{pre:sys-model}
The discrete-time dynamics of a CAV are modeled as
\begin{equation}
    \bm{x}_{k+1} = f(\bm{x}_k, \bm{u}_k)
    \label{eq:dynamic-eq}
\end{equation}
where the state $\bm{x}_k = [x_k, y_k, v_k, \theta_k]^T$ includes longitudinal and lateral positions, speed, and heading, respectively. The control input $\bm{u}_k = [a_k, \delta_k]^T$ comprises acceleration and steering. We adopt the kinematic bicycle model to discretize the dynamics:
\begin{equation}
    \begin{array}{c}
    % \bm{x}_{k+1} \\
    \begin{bmatrix} x_{k+1} \\ y_{k+1} \\ v_{k+1} \\ \theta_{k+1} \end{bmatrix}
    \end{array} = 
    \begin{array}{c}
    % \hat{f}(\bm{x}_k, \bm{u}_k) \\
    \begin{bmatrix}
        x_k + v_k\cos(\theta_k+\beta_k)\cdot T_s \\
        y_k + v_k\sin(\theta_k+\beta_k)\cdot T_s \\
        v_k + a_k\cdot T_s \\
        \theta_k + \dfrac{v_k\sin\beta_k}{l_r}\cdot T_s
    \end{bmatrix}
    \end{array}
    \label{eq:discrete-dynamic-evaluate-eq}
\end{equation}
where $T_s$ is the sampling period, $l_f$ and $l_r$ represent the distances from the front and rear wheels to the center of mass, and $\beta_k$ is the slip angle defined as $\beta_k=\arctan(\tan\delta_k\cdot l_r/(l_f+l_r))$. This model allows for iterative prediction of future vehicle states.

% \begin{figure}[tp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/fig1.pdf}
%     \caption{Kinematic bicycle model schematic diagram}
%     \label{fig:bysicle-model}
% \end{figure}

\subsection{Prescribed Performance Constraints}\label{pre:ppc}
To ensure asymptotic error convergence, the tracking error $e(t)$ can be constrained within a shrinking bound:
\begin{equation}
    -\sigma_L p(t) < e(t) < \sigma_R p(t)
    \label{eq:ppc-constraints}
\end{equation}
where the performance function $p(t)$ satisfies: 1) it is smooth, strictly positive, and monotonically decreasing; 2) $\underset{t\to0}{\lim}p(t)=p_0$, $\underset{t\to\infty}{\lim}p(t)=p_\infty$, with $p_0>p_\infty>0$. From \cite{buPrescribedPerformanceControl2023}, we utilize the form $p(t) = (p_0 - p_\infty)\mathrm{e}^{-\iota t} + p_\infty$, with decay rate $\iota \in [0,1]$. To incorporate PPC into controller design, the constrained error is transformed into an unconstrained one via $e(t) = \Xi(\zeta)p(t)$, where $\Xi(\zeta)$ is smooth, strictly increasing, bounded as $\Xi(\zeta) \in (-\sigma_L, \sigma_R)$ and given by:
\begin{equation}
    \Xi(\zeta) = \frac{\sigma_R \mathrm{e}^\zeta - \sigma_L \mathrm{e}^{-\zeta}}{\mathrm{e}^\zeta + \mathrm{e}^{-\zeta}}, \quad 
    \zeta = \frac{1}{2}\ln\frac{e(t)/p(t)+\sigma_L}{\sigma_R - e(t)/p(t)}.
    \label{eq:error-transformation-function}
\end{equation}

\subsection{Control Barrier Function} \label{pre:cbf}
For the discrete-time system~\eqref{eq:dynamic-eq}, consider the superlevel safety set $\mathcal{C}$ induced by a continuously differentiable function $h:\mathbb{R}^n\to\mathbb{R}$ as
\begin{equation}
    \begin{aligned}
        \mathcal{C}               &= \{\bm{x}\in\mathbb{R}^n \mid h(\bm{x}) \ge 0\}, \\ 
        \partial \mathcal{C}      &= \{\bm{x}\in\mathbb{R}^n \mid h(\bm{x}) = 0\}, \\ 
        \mathrm{Int}(\mathcal{C}) &= \{\bm{x}\in\mathbb{R}^n \mid h(\bm{x}) > 0\}.
    \end{aligned}
    \label{safe-set-defination}
\end{equation}
The function $h(\cdot)$ is defined as a discrete-time CBF~\cite{agrawalDiscreteControlBarrier2017} if it satisfies
\begin{equation}
    h(\bm{x}_{k+1}) - (1-\gamma_k)h(\bm{x}_k) \ge 0, \quad \gamma_k \in (0,1]
    \label{eq:cbf-condition-final}
\end{equation}
which guarantees the forward invariance of the safe set $\mathcal{C}$.  
By designing the control input $\bm{u}_k$ to satisfy~\eqref{eq:cbf-condition-final}, the system remains within $\mathcal{C}$ for all $t>0$ to ensure safety criteria.

\subsection{Problem Formulation} \label{pre:prob-form}
Consider a vehicle navigating a two-dimensional roundabout (see Fig.~\ref{fig:roundabout}), where other vehicles appear randomly. Let $I^{\mathrm{ov}}=\{i \mid i\in\mathbb{Z}_{\ge0}\}$ represent the index set of vehicles within the control zone. When a new vehicle enters the zone, it is assigned the smallest unused index $i_{\mathrm{new}}=\min\{i\in\mathbb{Z}_{\ge0} \mid i\notin I^{\mathrm{ov}}\}$. This index is subsequently removed when the vehicle exits, ensuring a dynamic mapping between indices and vehicles.

To achieve safe and efficient roundabout navigation, the ego vehicle is required to optimize three objectives: travel time, control effort, and safety. These objectives will later be incorporated into the RL reward and MPC optimization formulations.


\textit{Objective 1 (Minimum Travel Time):}
Minimize the travel time required for the ego vehicle to reach the destination. This objective is characterized by a positive stage objective function $r_1(\bm{x})$:
\begin{equation}
    J_1 = t_T - t_0 = \int_{t_0}^{+\infty} \delta(\bm{p}_\tau)\,\mathrm{d}\tau
    = \Phi\left[\int_{t_0}^{+\infty} r_1(\bm{x}_\tau)\,\mathrm{d}\tau\right],
    \label{cost-function-time}
\end{equation}
where $\bm{p}_\tau=(x_\tau,y_\tau)$ is the ego vehicle position, $\delta(\bm{p}_\tau)$ indicates whether the destination set $\mathcal{X}_T$ has been reached, and $\Phi(\cdot)$ is a strictly increasing mapping.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/fig3.pdf}
    \caption{Overview of RLTrajGen-PPMPC-CBF framework. The RL module (top left) maps observations from the environment (top right) to actions $(\bm{q}_t, \bm{w}_t)$. The action $\bm{q}_t$ is processed by the trajectory generator (bottom left) to construct Trajectory Generator $\mathcal{G}_t$ and produce a prediction sequence $\bm{z}_t^*$ of length $n_p$, which is then used to solve an MPC problem yielding $u^{\mathrm{MPC}_t}$. This control input is refined by the CBF module (bottom right) to obtain $u^{\mathrm{CBF}_t}$, which is applied to the environment to generate rewards for RL training.}
    \vspace{-15pt}
    \label{fig:framework}
\end{figure*}


\textit{Objective 2 (Minimum Energy Consumption):}
Minimize the control effort through the accumulated control cost:
\begin{equation}
    J_2 =\int_{t_0}^{t_T} C(\bm{u}_\tau)\,\mathrm{d}\tau,
    \label{cost-function-energy}
\end{equation}
where $C(\cdot)$ is a positive control cost function.


\textit{Objective 3 (Safety Penalty):}
Maintain a minimum safety distance $\delta$ from surrounding vehicles, i.e., $\mathrm{dist}(\bm{p}_t,\bm{p}^{\mathrm{ov}_i}_t)\ge\delta$. Safety violations are quantified by a positive stage penalty function $r_2(\bm{p},\bm{p}^{\mathrm{ov}})$:
\begin{equation}
    J_3 = \int_{t_0}^{t_T} r_2(\bm{p}_\tau,\bm{p}^{\mathrm{ov}_i}_\tau)\,\mathrm{d}\tau,
    \label{cost-function-safety-penal}
\end{equation}
where larger values of $r_2(\cdot)$ correspond to more severe safety violations.

Then the combined optimal control problem is formulated as follows:
\begin{equation}
    \begin{aligned}
    &\min_{\bm{x},\bm{u}}\ 
    \int_{t_0}^{+\infty}
    \Big[
    r_1(\bm{x}_\tau) + \big(C(\bm{u}_\tau) + r_2(\bm{p}_\tau,\bm{p}^{\mathrm{ov}_i}_\tau)\big) \delta(\bm{p}_\tau)
    \Big]\,\mathrm{d}\tau \\
    &s.t.\left\{\begin{array}{l}
    \bm{x}_\tau \in \mathcal{C}_{\mathrm{safe}} \\
    \bm{u}_{\min}\le \bm{u}\le \bm{u}_{\max}
    \end{array}\right.
    \end{aligned}
    \label{final-problem}
\end{equation}
where $u_{\min}$, $u_{\max}$ denote the lower and upper bounds of $\bm{u}$, respectively, and $\mathcal{C}_{\mathrm{safe}}$ denote the safety set for avoids collisions.

==> tabs/tab1.tex <==
\begin{tabular}{clc}
    \toprule
    Physical quantity           & Description                & Dimension          \\
    \midrule
    \textbf{Ego State}          &                            & $\mathbb{R}^9$     \\
    $v_t$                       & vehicle speed              & $\mathbb{R}^1$     \\
    $\delta_t$                  & steering angle             & $\mathbb{R}^1$     \\
    $u_{t-1}$                   & prev. throttle/brake       & $\mathbb{R}^1$     \\
    $\delta_{t-1}$              & prev. steering             & $\mathbb{R}^1$     \\
    $r_t$                       & yaw rate                   & $\mathbb{R}^1$     \\
    $\Delta \psi$               & heading diff. to lane      & $\mathbb{R}^1$     \\
    $d_L$                  & dist. to left lane line    & $\mathbb{R}^1$     \\
    $d_R$                 & dist. to right boundary    & $\mathbb{R}^1$     \\
    $p_{lat}$                   & lane lateral pos.          & $\mathbb{R}^1$     \\
    \midrule
    \textbf{Navigation}         &                            & $\mathbb{R}^{10}$  \\
    $d_{\parallel}$$\times$2    & proj. dist. (heading)      & $\mathbb{R}^1$     \\
    $d_{\perp}$$\times$2        & proj. dist. (lateral)      & $\mathbb{R}^1$     \\
    $R$$\times$2                & lane radius                & $\mathbb{R}^1$     \\
    $C$$\times$2                & turn dir. flag             & $\mathbb{R}^1$     \\
    $\theta$$\times$2           & lane angle                 & $\mathbb{R}^1$     \\
    \midrule
    \textbf{Surrounding}        &                            & $\mathbb{R}^{240}$ \\
    $\bm{s}^{sur}_t$        & surrounding LiDAR features & $\mathbb{R}^{240}$ \\
    \bottomrule
\end{tabular}



==> tabs/tab3.tex <==
\begin{tabular}{ccc}
    \toprule
    Name             & Description                   & Value   \\
    \midrule
    \textbf{Density} & Traffic density in the env    & 0.2     \\
    \textbf{Mode}    & Vehicle generation patterns   & respawn \\
    \textbf{Horizon} & Time of survival of the ego   & 1000    \\
    \bottomrule
\end{tabular}

==> tabs/tab4.tex <==
\begin{tabular}{ccc}
    \toprule
    Param        & Description             & Value             \\
    \midrule
    \textbf{RL}            &                         &                   \\
    $N_{\mathrm{epoch}}$   & epoch                   & $20$              \\
    $l_r$                  & learning rate           & $3\times10^{-4}$  \\
    $N_{\mathrm{sample}}$  & total sample steps      & $2\times10^6$     \\
    $N_{\mathrm{buffer}}$  & max buffer size         & $4096$            \\
    $\gamma$               & gamma                   & $0.99$            \\
    $\lambda$              & lambda                  & $0.2$             \\
    $\omega_{V}$           & value loss coef         & $0.5$             \\
    \midrule
    \textbf{MPC} &                         &                   \\
    $n_p$        & predicted steps         & $5$               \\
    $n_{\bm{u}}$ & control time domain     & $5$               \\
    $T_s$        & time interval           & $0.02\times 5$    \\
    \bottomrule
\end{tabular}

==> utils/inc.tex <==
\let\labelindent\relax\let\proof\relax\let\endproof\relax

\usepackage{amsmath,amssymb,amsfonts}
\usepackage{amsthm}
\usepackage{algorithmic}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{picinpar}
\usepackage{array}
\usepackage{stfloats}
\usepackage{url}
\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{enumitem}
\renewcommand{\arraystretch}{1.2}
% custom add
\usepackage{bm}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{colortbl}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}

% \captionsetup[table]{labelsep=period,textfont = sc}
% custom def
\newcommand{\Eqref}[1]{Eq.~\eqref{#1}}
\newcommand{\Secref}[1]{Sec.~\ref{#1}}
\newcommand{\Figref}[1]{Fig.~\ref{#1}}
\newcommand{\Tabref}[1]{Tab.~\ref{#1}}
% \newcommand{\Medref}[1]{\hyperref[method:#1]{#1}}
\newcommand{\Medref}[1]{%
  \hyperref[tab:methods]{\textcolor{blue}{#1}}%
}
\newcommand{\tablecaption}[1]{\caption{\textsc{#1}}}

\allowdisplaybreaks[4]

\usepackage{cite}
\makeatletter
\let\NAT@parse\undefined
\renewcommand{\@cite}[2]{\textcolor{blue}{[#1\if@tempswa , #2\fi]}}
\renewcommand{\eqref}[1]{\textcolor{blue}{\hyperref[#1]{(\ref*{#1})}}}
\makeatother
\usepackage[colorlinks=true, linkcolor=blue, citecolor=blue, urlcolor=blue]{hyperref}


